Analysing parameter space correlations of recent 13 TeV gluino and squark searches in the pMSSM

This paper examines unexplored correlations in the parameter spaces probed by recent ATLAS analyses for gluinos and squarks, addressing various shortcomings in the literature. Six 13 TeV ATLAS analyses based on 3.2 fb$^{-1}$ of integrated luminosity are interpreted in the 19-parameter R-parity conserving phenomenological minimal supersymmetric extension to the Standard Model (pMSSM). The distinct regions covered by each search are independent of prior, and we reveal particularly striking complementarity between the 2-6 jets and Multi-b searches. In the leptonic searches, we identify better sensitivity to models than those used for analysis optimisation, notably a squark-slepton-wino scenario for the SS/3L search. Further, we show how collider searches for coloured states probe the structure of the pMSSM dark sector more extensively than the Monojet analysis alone, with sensitivity to parameter spaces that are challenging for direct detection experiments.

==> body/lumi.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\subsection{\label{sec:lumi}Prospects for 30 and 300~fb$^{-1}$}

This section performs a simple estimate to characterise the effect of increasing luminosity on the sensitivity of models. 
We consider the subset of pMSSM points that have total strong production cross-section greater than 5~fb.
From these, those which are not excluded by 3.2~fb$^{-1}$ of integrated luminosity
had their expected yields scaled to higher luminosity, assuming a flat systematic uncertainty of 5\%.
We identify points that are not excluded by our interpretation of the six 13~TeV 3.2~fb$^{-1}$
points, and in addition remain below sensitivity for higher luminosity.
These points therefore would require novel techniques to bring into sensitivity, 
whose sensitivity is effectively `immune' to increased luminosity.

==> side/cutflows.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\label{sec:vali_cutflows}Cutflows}

Cutflows were provided in the supplementary material for each analysis considered in this work. First, we performed a cutflow validation against this material to ensure our implementations of each search in \textsc{MadAnalysis5} are selecting the correct kinematic space of events. We generated the simplified model signals to validate selections in all signal regions
used by ATLAS. This is done using the same Monte Carlo setup as all the pMSSM points simulated in this study (Subection~\ref{sec:13TeV_method}).

Tables~\ref{tab:cuflow_26J} to \ref{tab:cutflow_MonoJ} compares the public signal acceptances `ATLAS' after each selection criterion `Cut' with ours `MA5 Recast'. The variables used to label each cut in the cutflow tables are shown for completeness; please see the references in Table~\ref{tab:listSearches} for full definitions. Overall, we achieved better than 30\% agreement in the final yields for all signal regions `SR' of each analysis. This is reasonable given we used a different version of Pythia for showering compared with ATLAS, together with the same object isolation, overlap removal, reconstruction and $b$-tagging efficiencies in the \textsc{Delphes} detector simulation for all six analyses (to reduce disk usage to a manageable level). 



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{llll}
\toprule
					      & 											             &\multicolumn{2}{l}{Acceptance [\%]} \\
SR                   & Cut                                         & ATLAS          & MA5 Recast                \\
\midrule
\multirow{7}{*}{2jl} & Initial                                     & 100            & 100                          \\
                     & $E_{\rm T}^{\rm miss}, p_{\rm T}^{j1} > 200$ GeV 	    & 90.2           & 91.4                       \\
                     & 2 jet multiplicity                          & 90.2           & 91.4                    \\
                     & $\Delta \phi(E_{\rm T}^{\rm miss}, {\rm jet})_\textrm{min}$ & 55.0           & 56.1                       \\
                     & $p_{\rm T}^{j2}>200$ GeV                            & 54.3           & 54.9                       \\
                     & $E_{\rm T}^{\rm miss}/\sqrt{H_{\rm T}}>15$ GeV$^{1/2}$     & 29.2           & 28.7                       \\
                     & $m_{\rm eff}>1200$ GeV                      & 29.1           & 28.7                       \\
\midrule
\multirow{7}{*}{2jm} & Initial                                     & 100          & 100                      \\
                     & $E_{\rm T}^{\rm miss} > 200$, $p_{\rm T}^{j1} > 300$ GeV 	    & 89.8           & 90.6                       \\
                     & 2 jet multiplicity                          & 89.8           & 90.6                       \\
                     & $\Delta \phi(E_{\rm T}^{\rm miss}, {\rm jet})_\textrm{min}$ & 72.2           & 73.0                       \\
                     & $p_{\rm T}^{j2}>50$ GeV                           & 72.2           & 73.0                       \\
                     & $E_{\rm T}^{\rm miss}/\sqrt{H_{\rm T}}>15$ GeV$^{1/2}$      & 34.8           & 34.6                       \\
                     & $m_{\rm eff}>1600$ GeV                               & 34.3           & 33.7                       \\
\midrule
\multirow{7}{*}{2jt} & Initial                                     & 100          & 100                      \\
                     & $E_{\rm T}^{\rm miss}, p_{\rm T}^{j1} > 200$ GeV 	    & 90.2           & 91.4                       \\
                     & 2 jet multiplicity                          & 90.2           & 91.4                       \\
                     & $\Delta \phi(E_{\rm T}^{\rm miss}, {\rm jet})_\textrm{min}$ & 55.0           & 56.1                       \\
                     & $p_{\rm T}^{j2} > 200$ GeV                            & 54.3           & 54.9                       \\
                     & $E_{\rm T}^{\rm miss}/\sqrt{H_{\rm T}}>20$ GeV$^{1/2}$ & 16.7           & 16.2                       \\
                     & $m_{\rm eff} > 2000$ GeV                               & 16.0           & 14.8                       \\
\midrule
\multirow{9}{*}{4jt} & Initial                                     & 100          & 100                      \\
                     & $E_{\rm T}^{\rm miss}, p_{\rm T}^{j1} > 200$ GeV 	    & 90.2           & 91.4                       \\
                     & 4 jet multiplicity                          & 85.7           & 86.6                  \\
                     & $\Delta \phi(E_{\rm T}^{\rm miss}, {\rm jet})_\textrm{min}$ & 59.7           & 60.1                       \\
                     & $p_{\rm T}^{j2}>100$ GeV                            & 59.7           & 60.1                       \\
                     & $p_{\rm T}^{j4}>100$ GeV                            & 52.3           & 51.6                       \\
                     & Aplanarity $> 0.04$                                  & 35.6           & 35.9                       \\
                     & $E_{\rm T}^{\rm miss}/m_{\rm eff}>0.2$          & 25.2           & 26.4                       \\
                     & $m_{\rm eff}>2200$ GeV                               & 21.4           & 20.4                       \\
\midrule
\multirow{9}{*}{5j}  & Initial                                     & 100          & 100                      \\
                     & $E_{\rm T}^{\rm miss}, p_{\rm T}^{j1} > 200$ GeV 	    & 90.2           & 91.4                       \\
                     & 5 jet multiplicity                          & 64.3           & 67.3                       \\
                     & $\Delta \phi(E_{\rm T}^{\rm miss}, {\rm jet})_\textrm{min}$ & 43.6           & 45.3                       \\
                     & $p_{\rm T}^{j2}>100$ GeV                            & 43.6           & 45.3                       \\
                     & $p_{\rm T}^{j4}>100$ GeV                            & 40.2           & 41.4                       \\
                     & Aplanarity $> 0.04$                                 & 28.6           & 30.1                       \\
                     & $E_{\rm T}^{\rm miss}/m_{\rm eff}>0.25$          & 14.0           & 15.1                       \\
                     & $m_{\rm eff}>1600$ GeV                               & 13.9           & 14.8                       \\
\midrule
\multirow{9}{*}{6jm} & Initial                                     & 100          & 100                      \\
                     & $E_{\rm T}^{\rm miss}, p_{\rm T}^{j1} > 200$ GeV 	    & 90.2           & 91.4                       \\
                     & 6 jet multiplicity                          & 36.8           & 42.3                       \\
                     & $\Delta \phi(E_{\rm T}^{\rm miss}, {\rm jet})_\textrm{min}$ & 23.7           & 27.3                       \\
                     & $p_{\rm T}^{j2}>100$ GeV                            & 23.7           & 27.3                       \\
                     & $p_{\rm T}^{j4}>100$ GeV                            & 22.6           & 26.0                       \\
                     & Aplanarity $>0.04$                                 & 16.9           & 20.0                       \\
                     & $E_{\rm T}^{\rm miss}/m_{\rm eff}>0.25$          & 7.6            & 8.9                        \\
                     & $m_{\rm eff}>1600$ GeV                               & 7.5            & 8.8                        \\
\midrule
\multirow{9}{*}{6jt} & Initial                                     & 100          & 100                      \\
                     & $E_{\rm T}^{\rm miss}, p_{\rm T}^{j1} > 200$ GeV 	    & 90.2           & 91.4                       \\
                     & 6 jet multiplicity                          & 36.8           & 42.3                       \\
                     & $\Delta \phi(E_{\rm T}^{\rm miss}, {\rm jet})_\textrm{min}$ & 23.7           & 27.3                       \\
                     & $p_{\rm T}^{j2}>100$ GeV                            & 23.7           & 27.3                       \\
                     & $p_{\rm T}^{j4}>100$ GeV                            & 22.6           & 26.0                       \\
                     & Aplanarity $>0.04$                                  & 16.9           & 20.0                       \\
                     & $E_{\rm T}^{\rm miss}/m_{\rm eff}>0.2$          & 10.6           & 13.0                       \\
                     & $m_{\rm eff}>2000$ GeV                               & 9.9            & 11.9                       \\
\bottomrule
\end{tabular}
\caption{Cutflow comparison for 2--6 jets analysis using gluino direct decay $\left(m(\tilde{g}), m(\tilde{\chi}^0_1)\right) = (1600, 0)$ GeV signal.}
\label{tab:cuflow_26J}
\end{table}




\begin{table}[]
\centering
\begin{tabular}{llll}
\toprule
               & \multicolumn{2}{l}{Acceptance [\%]} \\
Cut            & ATLAS          & MA5 Recast            \\
\midrule
Initial & 100          & 100                      \\
Preselection   & 99.9           & --                         \\
Event cleaning & 99.0           & --                         \\
MET cleaning   & 95.8           & --                         \\
Lepton veto    & 47.8           & 48.8                       \\
\midrule\midrule
6j50           & 42.4           & 44.1                       \\
trigger        & 42.4           & --                         \\
\midrule
8j50           & 25.0           & 25.7                       \\
$E_{\rm T}^{\rm miss}/\sqrt{H_{\rm T}} > 4$ GeV$^{1/2}$  & 17.9           & 18.5                       \\
$N_\textrm{b-jet} \geq 0$        & 17.9           & 18.5                       \\
$N_\textrm{b-jet} \geq 1$        & 17.3           & 17.9                       \\
$N_\textrm{b-jet} \geq 2$        & 14.2           & 15.5                       \\
\midrule
9j50           & 16.5           & 16.6                       \\
$E_{\rm T}^{\rm miss}/\sqrt{H_{\rm T}} > 4$ GeV$^{1/2}$  & 11.3           & 11.6                       \\
$N_\textrm{b-jet} \geq 0$        & 11.3           & 11.6                       \\
$N_\textrm{b-jet} \geq 1$        & 11.0           & 11.3                       \\
$N_\textrm{b-jet} \geq 2$        & 9.3            & 10.1                       \\
\midrule
10j50          & 9.1            & 9.3                        \\
$E_{\rm T}^{\rm miss}/\sqrt{H_{\rm T}} > 4$ GeV$^{1/2}$  & 6.0            & 6.2                        \\
$N_\textrm{b-jet} \geq 0$        & 6.0            & 6.2                        \\
$N_\textrm{b-jet} \geq 1$        & 5.8            & 6.1                        \\
$N_\textrm{b-jet} \geq 2$        & 5.1            & 5.5                        \\
\midrule\midrule
5j80           & 40.5           & 43.5                       \\
trigger        & 40.5           & --                         \\
\midrule
7j80           & 19.7           & 18.7                       \\
$E_{\rm T}^{\rm miss}/\sqrt{H_{\rm T}} > 4$ GeV$^{1/2}$  & 13.6           & 13.2                       \\
$N_\textrm{b-jet} \geq 0$        & 13.6           & 13.2                       \\
$N_\textrm{b-jet} \geq 1$        & 13.2           & 12.8                       \\
$N_\textrm{b-jet} \geq 2$        & 10.8           & 11.1                       \\
\midrule
8j80           & 10.3           & 9.7                        \\
$E_{\rm T}^{\rm miss}/\sqrt{H_{\rm T}} > 4$ GeV$^{1/2}$  & 6.8            & 6.6                        \\
$N_\textrm{b-jet} \geq 0$        & 6.8            & 6.6                        \\
$N_\textrm{b-jet} \geq 1$        & 6.7            & 6.4                        \\
$N_\textrm{b-jet} \geq 2$        & 5.5            & 5.8                        \\
\bottomrule
\end{tabular}
\caption{Cutflow comparison for 7--10 jets analysis using pMSSM slice signal. Signal regions are defined by the jet multiplicities and b-tagging requirements.}
\label{tab:cutflow_710J}
\end{table}



\begin{table}[]
\centering
\begin{tabular}{llll}
\toprule 
                           &                              & \multicolumn{2}{l}{Acceptance [\%]} \\
SR                         & Cuts                         & ATLAS             & MA5 Recast                 \\
\midrule\midrule
   \multicolumn{4}{l}{Gluino 1-step $\left(m(\tilde{g}), m(\tilde{\chi}^\pm_1), m(\tilde{\chi}^0_1)\right) = (1385, 705, 25)$ GeV} \\
\midrule
\multirow{8}{*}{Preselect} & Initial                        & 100             & 100                             \\
                           & Cleaning cuts                  & 88.5              & --                                \\
                           & 1 base lepton                  & 30.8              & 29.8                              \\
                           & 1 signal lepton                & 25.1              & 26.5                              \\
                           & $N_\textrm{jet} \geq 3$        & 25.1              & 26.5                              \\
                           & $E_{\rm T}^{\rm miss} > 100$ GeV  & 24.6              & 25.5                              \\
                           & $E_{\rm T}^{\rm miss}$ trigger & 24.4              & --                                \\
                           & $p_{\rm T}^\ell >  35 $ GeV       & 23.3              & 25.5                              \\
\midrule
\multirow{8}{*}{5j}        & $E_{\rm T}^{\rm miss} > 250$ GeV & 19.2              & 20.6                              \\
                           & $N_\textrm{jet} \geq 5$       & 18.2              & 19.7                              \\
                           & $p_{\rm T}^{j1} > 225$ GeV       & 18.2              & 19.4                              \\
                           & $p_{\rm T}^{j5} > 50$ GeV        & 16.0              & 16.9                              \\
                           & Aplanarity $>0.04$ 		     & 12.7              & 13.0                              \\
                           & $m_{\rm T} > 275$ GeV            & 8.5               & 8.5                               \\
                           & $E_{\rm T}^{\rm miss}/m_{\rm eff} > 0.1$  & 8.3   & 8.4                             \\
                           & $m_{\rm eff} > 1800$ GeV         & 7.6               & 7.2                               \\
\midrule
\multirow{8}{*}{6j}        & $E_{\rm T}^{\rm miss} > 250$ GeV  & 19.2              & 20.6                              \\
                           & $N_\textrm{jet} \geq 6$     	& 15.1              & 17.5                              \\
                           & $p_{\rm T}^{j1} > 125$ GeV        & 15.1              & 17.5                              \\
                           & $p_{\rm T}^{j6} > 30$ GeV         & 15.1              & 16.5                              \\
                           & Aplanarity $>0.04$ 			   & 12.0              & 12.8                              \\
                           & $m_{\rm T} > 225 $ GeV         	& 9.0               & 9.2                               \\
                           & $E_{\rm T}^{\rm miss}/m_{\rm eff} > 0.2$  & 5.3       & 5.5                           \\
                           & $m_{\rm eff} > 1000$ GeV       	& 5.3               & 5.5                               \\
\midrule
\multirow{7}{*}{4j low-x}  & $E_{\rm T}^{\rm miss} > 200$ GeV  & 21.6              & 22.5                              \\
                           & $N_\textrm{jet} \geq 4$      	& 21.4              & 22.4                              \\
                           & $p_{\rm T}^{j1} > 325$ GeV        & 19.4              & 19.1                              \\
                           & $p_{\rm T}^{j4} > 150$ GeV        & 10.5              & 10.3                              \\
                           & Aplanarity $ >0.04$ 			   & 8.9               & 8.4                               \\
                           & $m_{\rm T} > 125 $ GeV         	& 7.7               & 6.9                               \\
                           & $m_{\rm eff} > 2000$ GeV      	   & 6.3               & 5.9                               \\
\midrule
\multirow{7}{*}{4j high-x} & $E_{\rm T}^{\rm miss} > 200$ GeV  & 21.6              & 22.5                              \\
                           & $N_\textrm{jet} \geq 4$   		   & 21.4              & 22.4                              \\
                           & $p_{\rm T}^{j1} > 325$ GeV       	& 19.4              & 19.1                              \\
                           & $p_{\rm T}^{j4} > 30$ GeV       	& 19.4              & 19.1                              \\
                           & $m_{\rm T} > 425$ GeV         		& --                & 7.6                               \\
                           & $E_{\rm T}^{\rm miss}/m_{\rm eff} > 0.3 $   & 1.5       & 1.5                        \\
                           & $m_{\rm eff} > 1800 $ GeV         & 1.4               & 1.3                               \\
\midrule\midrule
   \multicolumn{4}{l}{Gluino 1-step $\left(m(\tilde{g}), m(\tilde{\chi}^\pm_1), m(\tilde{\chi}^0_1)\right) = (1000, 110, 60)$ GeV} 								\\
\midrule
\multirow{7}{*}{Preselect} & Initial                          & 100             & 100                             \\
                           & Cleaning cuts                    & 85.9              & --                                \\
                           & 1 base lepton                    & 36.2              & --                                \\
                           & 1 signal lepton                  & 30.3              & 35.1                             \\
                           & $N_\textrm{jet} \geq 2$          & 30.3              & 26.5                             \\
                           & $p_{\rm T}^\ell < 35 $ GeV       & 9.9               & 9.4                              \\
                           & $E_{\rm T}^{\rm miss} > 200$ GeV & 6.8               & 6.5                              \\
\midrule
\multirow{5}{*}{2j}        & $E_{\rm T}^{\rm miss} > 530$ GeV  & 0.8               & 0.9                              \\
                           & $N_\textrm{jet} \geq 2$           & 0.8               & 0.9                              \\
                           & $p_{\rm T}^{j1} > 180$ GeV        & 0.8               & 0.9                              \\
                           & $m_{\rm T} > 100$ GeV           	& 0.2               & 0.2                              \\
                           & $E_{\rm T}^{\rm miss}/m_{\rm eff} > 0.3$     & 0.0               & 0.03                              \\
\midrule
\multirow{7}{*}{5j}        & $E_{\rm T}^{\rm miss} > 375$ GeV & 2.5               & 2.6                              \\
                           & $N_\textrm{jet} \geq 5$          & 2.3               & 2.6                              \\
                           & $p_{\rm T}^{j1} > 200$ GeV       & 2.3               & 2.4                              \\
                           & $p_{\rm T}^{j2} > 200$ GeV       & 2.1               & 2.4                              \\
                           & $p_{\rm T}^{j3} > 200$ GeV       & 1.4               & 2.1                              \\
                           & Aplanarity $> 0.02$ 		        & 1.3               & 1.4                              \\
                           & $H_{\rm T} > 1100$ GeV           & 1.2               & 1.3                             	\\
\bottomrule
\end{tabular}

\caption{Cutflow comparison for 1 lepton analysis.}
\label{tab:cutflow_1L}
\end{table}


\begin{table}[]
\centering
\begin{tabular}{lllll}
\toprule
                                  &                                  & \multicolumn{2}{l}{Acceptance [\%]} \\
SR                                & Cut                         		& ATLAS       & MA5 Recast            \\
\midrule\midrule
   \multicolumn{4}{c}{Gtt $\left(m(\tilde{g}), m(\tilde{\chi}^0_1)\right) = (1700, 200)$ GeV}                       \\
\midrule
\multirow{6}{*}{Preselect}        & Initial               		 		& 100       & 100                   \\
                                  & Trigger                      		& 92.1        & --                    \\
                                  & Cleaning                     		& 90.7        & --                    \\
                                  & $N_\textrm{jets} \geq 4$     		& 90.7        & 94.5                  \\
                                  & $N_\textrm{b-jets} \geq 3$   		& 68.2        & 70.3                  \\
                                  & $E_\textrm{T}^{\rm miss} > 200$ GeV    & 63.5        & 63.9                  \\
\midrule                              
\multirow{4}{*}{Gtt-0L} 		  & Lepton veto                  		& 35.2        & 34.7                  \\
                                  & $\Delta \phi^{4j}_{\rm min}$ 		& 26.3        & 26.1                  \\
                                  & $N_\textrm{jets} \geq 8$  & 22.0    & 22.5                  \\
                                  & $m_\textrm{T, min}^\textrm{b-jets} > 80$ GeV & 19.8        & 20.2                  \\
\midrule
\multirow{4}{*}{Gtt-0L-A}         & $m_{\rm eff}^{\rm incl} > 1700$ GeV		& 18.5        & 18.7                  \\
                                  & $E_\textrm{T}^{\rm miss} > 400 $ GeV   & 15.4        & 15.4                  \\
                                  & $N_\textrm{b-jets} \geq 3$    		& 15.4        & 15.4                  \\
                                  & $N_\textrm{top} \geq 1$             & 15.2        & 14.4                  \\
\midrule
\multirow{4}{*}{Gtt-0L-B}         & $m_{\rm eff}^{\rm incl} > 1250$ GeV		& 19.7        & 20.0                  \\
                                  & $E_\textrm{T}^{\rm miss} > 350 $ GeV   & 17.2        & 17.3                  \\
                                  & $N_\textrm{b-jets} \geq 4$     		& 11.1        & 11.4                  \\
                                  & $N_\textrm{top} \geq 1$             & 10.9        & 10.9                  \\
\midrule
\multirow{3}{*}{Gtt-0L-C}         & $m_{\rm eff}^{\rm incl} > 1250$ GeV		& 19.7        & 20.0                  \\
                                  & $E_\textrm{T}^{\rm miss} > 350 $ GeV   & 17.2        & 17.3                  \\
                                  & $N_\textrm{b-jets} \geq 4$      	& 11.1        & 11.4                  \\
\midrule
\multirow{4}{*}{Gtt-1L} 		    & 1 signal lepton                		& 28.3        & 29.2                  \\
                                  & $N_\textrm{b-jets} \geq 6$   		& 26.5        & 27.7                  \\
                                  & $m_\textrm{T, min}^\textrm{b-jets} > 80$ GeV & 17.1        & 17.8                  \\
                                  & $m_{\rm T} > $ 150 GeV         		& 14.2        & 14.7                  \\
\midrule
\multirow{3}{*}{Gtt-1L-A}         & $m_{\rm eff}^{\rm incl} > 1100$ GeV	& 14.2        & 14.7                  \\
                                  & $E_\textrm{T}^{\rm miss} > 200$ GeV    & 14.2        & 14.7                  \\
                                  & $N_\textrm{top} \geq 1$             & 13.5        & 13.6                  \\
\midrule
\multirow{2}{*}{Gtt-1L-B}         & $m_{\rm eff}^{\rm incl} > 1100$ GeV	& 14.2        & 14.7                  \\
                                  & $E_\textrm{T}^{\rm miss} > 300$ GeV    & 13.3        & 13.8                  \\
\midrule\midrule
   \multicolumn{4}{c}{Gbb $\left(m(\tilde{g}), m(\tilde{\chi}^0_1)\right) = (1700, 200)$ GeV} \\
\midrule
\multirow{6}{*}{Preselect}        & Initial               		 		& 100       & 100                \\
                                  & Trigger                      		& 96.0        & --                 \\
                                  & Cleaning                     		& 94.7        & --                   \\
                                  & $N_\textrm{jets} \geq 4$     		& 92.1        & 92.2                 \\
                                  & $N_\textrm{b-jets} \geq 3$   		& 58.9        & 60.4                 \\
                                  & $E_\textrm{T}^{\rm miss} > 200$ GeV    & 55.6        & 55.6                 \\
\midrule
\multirow{2}{*}{Gbb-0L}           & Lepton veto                  		& 55.0        & 55.6                 \\
                                  & $\Delta \phi^{4j}_{\rm min}$ 		& 39.5        & 40.6                 \\
\midrule
\multirow{4}{*}{Gbb-0L-A}         & $m_{\rm eff}^{4j} > 1600$ GeV   		& 36.6        & 36.3                 \\
                                  & $E_\textrm{T}^{\rm miss} > 350$ GeV    & 33.0        & 32.5                 \\
                                  & $N_\textrm{jets}^{p_{\rm T} > 90} \geq 4$   & 29.4        & 29.1                 \\
                                  & $N_\textrm{b-jets}^{p_{\rm T} > 90} \geq 3$ & 25.5        & 24.9                 \\
\midrule
\multirow{4}{*}{Gbb-0L-B}         & $m_{\rm eff}^{4j} > 1400$ GeV   		& 38.5     	 & 38.8                 \\
                                  & $E_\textrm{T}^{\rm miss} > 450$ GeV        & 30.2        & 30.1                 \\
                                  & $N_\textrm{jets}^{p_{\rm T} > 90} \geq 4$   & 26.7        & 26.6                 \\
                                  & $N_\textrm{b-jets}^{p_{\rm T} > 90} \geq 3$ & 23.1        & 22.7                 \\
\midrule
\multirow{2}{*}{Gbb-0L-C}         & $m_{\rm eff}^{4j} > 1400$ GeV   		& 38.5        & 38.8                 \\
                                  & $E_\textrm{T}^{\rm miss} > 300$ GeV    & 28.1        & 27.6                 \\
\bottomrule
\end{tabular}

\caption{Cutflow comparison for Multi-b analysis.}
\label{tab:cutflow_Multib}
\end{table}





\begin{table}[]
\centering
\begin{tabular}{llll}
\toprule
                        &                  				     & \multicolumn{2}{l}{Acceptance [\%]}           \\
SR                      & Cut             				     & ATLAS          & MA5 Recast                \\
\midrule\midrule
   \multicolumn{4}{c}{Gluino slepton $\left(m(\tilde{g}), m(\tilde{\chi}^0_1)\right) = (1300, 500)$ GeV} \\
\midrule
\multirow{7}{*}{SR0b3j} & Initial          				     & 100            & 100                    \\
                        & $N_{\ell}\geq3$  				     & 9.7            & 10.1                     \\
                        & Trigger          				     & 9.7            & --                       \\
                        & $N_\textrm{b-jet}=0$ & 7.9       & 8.6                       \\
                        & $N_\textrm{jet}\geq3$& 7.4       & 8.1                       \\
                        & $E_{\rm T}^{\rm miss} > 200$ GeV & 5.1            & 5.9                      \\
                        & $m_{\rm eff} > 550$ GeV          & 5.1            & 5.9                      \\
\midrule\midrule
   \multicolumn{4}{c}{Gluino 2-step $\left(m(\tilde{g}), m(\tilde{\chi}^0_1)\right) = (1100, 400)$ GeV}   \\
\midrule
\multirow{7}{*}{SR0b5j} & Initial          				     & 100            & 100                    \\
                        & $N_{\ell}^{\rm SS}\geq2$  	     & 3.6   		    & 3.9                      \\
                        & Trigger          				     & 3.4            & --                       \\
                        & $N_\textrm{b-jet}=0$& 2.2        & 2.5                       \\
                        & $N_\textrm{jet}\geq5$& 1.5       & 2.0                       \\
                        & $E_{\rm T}^{\rm miss} > 125$ GeV & 1.3            & 1.6                      \\
                        & $m_{\rm eff} > 650$ GeV          & 1.3            & 1.6                      \\
\midrule\midrule 
   \multicolumn{4}{c}{Sbottom 1-step $\left(m(\tilde{b}_1), m(\tilde{\chi}^0_1)\right) = (600, 50)$ GeV}     \\
\midrule
\multirow{7}{*}{SR1b}   & Initial          				     & 100            & 100                    \\
                        & $N_{\ell}^{\rm SS}\geq2$  	     & 4.6    		    & 4.68                     \\
                        & Trigger          				     & 4.1            & --                       \\
                        & $N_\textrm{b-jet}\geq1$   	     & 3.6            & 3.92                     \\
                        & $N_\textrm{jet}\geq4$     	     & 2.0            & 2.31                     \\
                        & $E_{\rm T}^{\rm miss} > 150$ GeV & 1.3            & 1.44                     \\
                        & $m_{\rm eff} > 550$ GeV          & 1.3            & 1.44                     \\
\midrule\midrule
   \multicolumn{4}{c}{Gtt $\left(m(\tilde{g}), m(\tilde{\chi}^0_1)\right) = (1200, 700)$ GeV}        \\
\midrule
\multirow{6}{*}{SR3b}   & Initial          				     & 100            & 100                    \\
                        & $N_{\ell}^{\rm SS}\geq2$ 	     & 3.4   		    & 3.6                      \\
                        & Trigger          				     & 3.1            & --                       \\
                        & $N_\textrm{b-jet}\geq3$		     & 1.5            & 1.8                      \\
                        & $E_{\rm T}^{\rm miss} > 125$ GeV & 1.2            & 1.4                      \\
                        & $m_{\rm eff} > 650$ GeV          & 1.2            & 1.4                      \\
\bottomrule
\end{tabular}

\caption{Cutflow comparison for SS/3L analysis.}
\label{tab:cutflow_SS3L}
\end{table}





\begin{table}[]
\centering
\begin{tabular}{llll}
\toprule
                           &                                        & \multicolumn{2}{l}{Acceptance [\%]} \\
SR                         & Cut                                    & ATLAS            & MA5 Recast           \\
\midrule
\multirow{9}{*}{Preselect} & Initial events                         & 100            & 100                \\
                           & Trigger                                & 83.7           & --                   \\
                           & Cleaning cut                           & 83.0           & --                   \\
                           & Lepton veto                            & 83.0           & 100                \\
                           & $N_{\rm jets} \leq 4$                  & 77.3           & 93.8               \\
                           & $\Delta \phi(E_{\rm T}^{\rm miss}, {\rm jet}) > 0.4$         & 73.5           & 88.4               \\
                           & Jet quality                            & 70.1           & --                   \\
                           & $p_{\rm T}^{j1} > 250$ GeV         & 22.7           & 18.8               \\
                           & $E_{\rm T}^{\rm miss} > 250$           & 21.1           & 16.7               \\
\midrule
EM1                        & $250 < E_{\rm T}^{\rm miss} < 300$ GeV & 3.0            & 2.4                \\
EM2                        & $300 < E_{\rm T}^{\rm miss} < 350$ GeV & 3.4            & 2.5                \\
EM3                        & $350 < E_{\rm T}^{\rm miss} < 400$ GeV & 3.1            & 2.6                \\
EM4                        & $400 < E_{\rm T}^{\rm miss} < 500$ GeV & 4.4            & 4.0                \\
EM5                        & $500 < E_{\rm T}^{\rm miss} < 600$ GeV & 2.8            & 2.4                \\
EM6                        & $600 < E_{\rm T}^{\rm miss} < 700$ GeV & 1.8            & 1.2                \\
IM7                        & $E_{\rm T}^{\rm miss} > 700$       GeV & 2.6            & 1.5               \\
\bottomrule
\end{tabular}
\caption{Cutflow comparison for Monojet analysis using the squark direct decay model using the $\left(m(\tilde{q}), m(\tilde{\chi}^0_1)\right) = (650, 645)$ GeV signal.}
\label{tab:cutflow_MonoJ}
\end{table}

